3D Part Assembly Generation with Instance Encoded Transformer

It is desirable to enable robots capable of automatic assembly. Structural understanding of object parts plays a crucial role in this task yet remains relatively unexplored. In this paper, we focus on the setting of furniture assembly from a complete set of part geometries, which is essentially a 6-DoF part pose estimation problem. We propose a multi-layer transformer-based framework that involves geometric and relational reasoning between parts to update the part poses iteratively. We carefully design a unique instance encoding to solve the ambiguity between geometrically-similar parts so that all parts can be distinguished. In addition to assembling from scratch, we extend our framework to a new task called in-process part assembly. Analogous to furniture maintenance, it requires robots to continue with unfinished products and assemble the remaining parts into appropriate positions. Our method achieves far more than 10% improvements over the current state-of-the-art in multiple metrics on the public PartNet dataset. Extensive experiments and quantitative comparisons demonstrate the effectiveness of the proposed framework.

==> tables/gnn_rebuttal.tex <==
\setlength{\tabcolsep}{3mm}
\small 
\centering
\begin{tabular}{c|c|c|c|c}
arch & w/ins-enc? & SCD $\downarrow$ & PA $\uparrow$ & CA $\uparrow$ \\
\Xhline{2\arrayrulewidth}
\rule{0pt}{1.1\normalbaselineskip}
\multirow{2}*{GNN} & ~ & 0.0068 & 46.44 & 33.77 \\
~ & \cmark & 0.0063 & 58.14 \color{blue}{(+11.70)} & 43.19 \color{blue}{(+9.42)} \\
\hline
\rule{0pt}{1.0\normalbaselineskip}
\multirow{2}*{Transformer} & ~ & 0.0068 & 48.40 & 36.04 \\
~ & \cmark & \textbf{0.0054} & \textbf{62.80} \color{blue}{(+14.40)} & \textbf{48.45} \color{blue}{(+12.41)} \\
\end{tabular}
